Metric for attractor overlap

We present the first general metric for attractor overlap (MAO) facilitating an unsupervised comparison of flow data sets. The starting point is two or more attractors, i.e., ensembles of states representing different operating conditions. The proposed metric generalizes the standard Hilbert-space distance between two snapshots to snapshot ensembles of two attractors. A reduced-order analysis for big data and many attractors is enabled by coarse-graining the snapshots into representative clusters with corresponding centroids and population probabilities. For a large number of attractors, MAO is augmented by proximity maps for the snapshots, the centroids, and the attractors, giving scientifically interpretable visual access to the closeness of the states. The coherent structures belonging to the overlap and disjoint states between these attractors are distilled by few representative centroids. We employ MAO for two quite different actuated flow configurations: (1) a two-dimensional wake of the fluidic pinball with vortices in a narrow frequency range and (2) three-dimensional wall turbulence with broadband frequency spectrum manipulated by spanwise traveling transversal surface waves. MAO compares and classifies these actuated flows in agreement with physical intuition. For instance, the first feature coordinate of the attractor proximity map correlates with drag for the fluidic pinball and for the turbulent boundary layer. MAO has a large spectrum of potential applications ranging from a quantitative comparison between numerical simulations and experimental particle-image velocimetry data to the analysis of simulations representing a myriad of different operating conditions.

==> S0_Shortened.tex <==
\begin{abstract}
We present the first general metric for attractor overlap (MAO) 
facilitating an unsupervised comparison of flow data sets.
The starting point is two or more attractors, 
i.e., ensembles of states representing different operating conditions.
The proposed metric generalizes the standard Hilbert-space distance
between two snapshots to snapshot ensembles of two attractors.
A reduced-order analysis for big data and many attractors
is enabled by coarse-graining the snapshots 
into  representative clusters
with corresponding centroids and population probabilities.
For a large number of attractors,
MAO is augmented by proximity maps for the snapshots, the centroids, and the attractors,
giving scientifically interpretable visual access to the closeness of the states.
The coherent structures
belonging to the overlap and disjoint states between these attractors 
are distilled by few representative centroids.
We employ MAO for two quite different actuated flow configurations:
(1) a two-dimensional wake of the fluidic pinball with vortices in a narrow frequency range
and (2) three-dimensional wall turbulence with broadband frequency spectrum 
manipulated by spanwise traveling transversal surface waves.
MAO compares and classifies these actuated flows in agreement with physical intuition.
For instance, the first feature coordinate of the attractor proximity map 
correlates with drag for the fluidic pinball and for the turbulent boundary layer.
MAO has a large spectrum of potential applications
ranging from   a quantitative comparison between numerical simulations and experimental particle-image velocimetry data
to the analysis of simulations representing a myriad of different operating conditions.
\end{abstract}


==> S4_Fig01.tex <==
%----- Figure ----------------------------------------------------------
\begin{figure}
	\centering
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid1}
		\put(1,36){\fbox{\tiny$ 1$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid11}
		\put(1,36){\fbox{\tiny$11$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid21}
		\put(1,36){\fbox{\tiny$21$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid31}
		\put(1,36){\fbox{\tiny$31$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid41}
		\put(1,36){\fbox{\tiny$41$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid2}
		\put(1,36){\fbox{\tiny$ 2$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid12}
		\put(1,36){\fbox{\tiny$12$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid22}
		\put(1,36){\fbox{\tiny$22$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid32}
		\put(1,36){\fbox{\tiny$32$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid42}
		\put(1,36){\fbox{\tiny$42$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid3}
		\put(1,36){\fbox{\tiny$ 3$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid13}
		\put(1,36){\fbox{\tiny$13$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid23}
		\put(1,36){\fbox{\tiny$23$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid33}
		\put(1,36){\fbox{\tiny$33$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid43}
		\put(1,36){\fbox{\tiny$43$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid4}
		\put(1,36){\fbox{\tiny$4$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid14}
		\put(1,36){\fbox{\tiny$14$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid24}
		\put(1,36){\fbox{\tiny$24$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid34}
		\put(1,36){\fbox{\tiny$34$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid44}
		\put(1,36){\fbox{\tiny$44$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid5}
		\put(1,36){\fbox{\tiny$5$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid15}
		\put(1,36){\fbox{\tiny$15$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid25}
		\put(1,36){\fbox{\tiny$25$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid35}
		\put(1,36){\fbox{\tiny$35$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid45}
		\put(1,36){\fbox{\tiny$45$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid6}
		\put(1,36){\fbox{\tiny$6$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid16}
		\put(1,36){\fbox{\tiny$16$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid26}
		\put(1,36){\fbox{\tiny$26$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid36}
		\put(1,36){\fbox{\tiny$36$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid46}
		\put(1,36){\fbox{\tiny$46$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid7}
		\put(1,36){\fbox{\tiny$7$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid17}
		\put(1,36){\fbox{\tiny$17$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid27}
		\put(1,36){\fbox{\tiny$27$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid37}
		\put(1,36){\fbox{\tiny$37$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid47}
		\put(1,36){\fbox{\tiny$47$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid8}
		\put(1,36){\fbox{\tiny$8$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid18}
		\put(1,36){\fbox{\tiny$18$}}
	\end{overpic}		
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid28}
		\put(1,36){\fbox{\tiny$28$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid38}
		\put(1,36){\fbox{\tiny$38$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid48}
		\put(1,36){\fbox{\tiny$48$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid9}
		\put(1,36){\fbox{\tiny$9$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid19}
		\put(1,36){\fbox{\tiny$19$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid29}
		\put(1,36){\fbox{\tiny$29$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid39}
		\put(1,36){\fbox{\tiny$39$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid49}
		\put(1,36){\fbox{\tiny$49$}}
	\end{overpic}\\
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid10}
		\put(1,36){\fbox{\tiny$10$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid20}
		\put(1,36){\fbox{\tiny$20$}}
	\end{overpic}	
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid30}
		\put(1,36){\fbox{\tiny$30$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid40}
		\put(1,36){\fbox{\tiny$40$}}
	\end{overpic}
	\begin{overpic}[width=2.5cm, trim=5.7cm 2.25cm 4.cm 0, clip=true]{Centroids/VorticityCentroid50}
		\put(1,36){\fbox{\tiny$50$}}
	\end{overpic}			
	\caption{Cluster centroids: All centroids that are visited during phase 1, and additional centroids for all other phases, that are exhibit strongly different features. Maybe in total: 4x5 or 5x4}
\label{Fig:Centroids}
\end{figure}
%----- End of figure ---------------------------------------------------



==> SX.tex <==
\section{Comments}
\subsection{On the title---Email of 2017-09-16}
I suggest that we give the paper a short \& concise title,
like  \emph{Metric for attractor overlap} (later abbreviated as MAO).

The reason for the short title is obvious.
Many famous papers like \emph{On the nature of turbulence} have short titles.

As per our last discussions,  \emph{Metric for attractor overlap}
shall become the branding of Rishabh's algorithm.

We can easily define such a metric without clusters and without entropy
and get something  very similar. Hence, putting clusters and entropy in the title is probably counter-advised.

Note that our MAO term is actuatually not inclusive enough.
It is actually a metric for snapshot ensemble overlap.
(1) We can also compare transients.
For most applications, this is a side aspect.
(2) Moreover, we have more than a metric (Jensen-Shannon entropy).
We also include visualization algorithms.
Again, I would argue that these are again side aspects of our approach.

\textcolor{red}{\bf 
BERND: Include Eurika's references that the JS entropy (square root) defines a metric
$$d(A,B) + d(B,C) \le d(A,C)$$.
}

